Shared-Endpoint Correlations and Hierarchy in Random Flows on Graphs

We analyze the correlation between randomly chosen edge weights on neighboring edges in a directed graph. This shared-endpoint correlation controls the expected organization of randomly drawn edge flows when the flow on each edge is conditionally independent of the flows on other edges given its endpoints. To model different relationships between endpoints and flow, we draw edge weights in two stages. First, assign a random description to the vertices by sampling random attributes at each vertex. Then, sample a Gaussian process (GP) and evaluate it on the pair of endpoints connected by each edge. We model different relationships between endpoint attributes and flow by varying the kernel associated with the GP. We then relate the expected flow structure to the smoothness class containing functions generated by the GP. We compute the exact shared-endpoint correlation for the squared exponential kernel and provide accurate approximations for Mat\'ern kernels. In addition, we provide asymptotics in both smooth and rough limits and isolate three distinct domains distinguished by the regularity of the ensemble of sampled functions. Taken together, these results demonstrate a consistent effect; smoother functions relating attributes to flow produce more organized flows.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
